Reduced rank extrapolation for multi-term Sylvester equations

We investigate the acceleration of stationary iterations for multi-term Sylvester equation by means of reduced rank extrapolation (RRE). Theoretical convergence results and implementations are provided for both small and large-scale problems. For the large-scale problems, an inexact non-stationary iteration is discussed, which makes use of low-rank matrix approximations. Numerical experiments illustrate the potential of the RRE acceleration which often leads to a substantial gain in convergence speed and therefore reducing the consumption of storage and computing time.

==> macros.tex <==
% ---------individual packages and formats---------
\usepackage{orcidlink}

\usepackage{amsmath, amscd, amssymb, amsthm, mathrsfs, mathtools}
\usepackage{array, booktabs, makecell} % for column headers
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\usepackage[american]{babel}
\usepackage{enumerate}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{soul}
\usepackage{tikz}
\usepackage[backgroundcolor=violet!60,textcolor=white,linecolor=gray]{todonotes}
\usepackage{xspace} % In-text comments
\usepackage{pgfplots, pgfplotstable}
\usepackage[normalem]{ulem}
\usepackage{multirow}
\usepackage{siunitx}

\RequirePackage[table]{xcolor}

%\usepackage[dvipsnames]{xcolor}

\pgfplotstableset{%
col sep = comma,
%row sep = newline,
%format = file
}
\pgfplotsset{
compat=1.18,
unbounded coords=jump,
x label style={font=\small},
y label style={font=\small},
x tick label style={font=\footnotesize},
y tick label style={font=\footnotesize}
}

% Algorithms
\usepackage[algosection,vlined,algo2e,linesnumbered,algoruled]{algorithm2e}
\SetKwComment{Comment}{}{}
\SetKwProg{Fn}{Function}{}{end}
\DontPrintSemicolon{}
\newcommand{\algcmd}[1]{\ensuremath{\text{\textbf{\em {#1\ }}}}}
\newcommand{\algdownto}{\algcmd{down\ to}}
\newcommand{\algnot}{\algcmd{not}}
\newcommand{\algand}{\algcmd{and}}
\newcommand{\algor}{\algcmd{or}}
\newcommand{\algto}{\algcmd{to}}
\newcommand{\algtrue}{\ensuremath{\text{\textbf{true}}}}
\newcommand{\algfalse}{\ensuremath{\text{\textbf{false}}}}

% numbering equations, tables, and figures by sections
\numberwithin{equation}{section}
\numberwithin{table}{section}
\numberwithin{figure}{section}

% theorems
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
%\theoremstyle{remark}
\newtheorem{remark}{Remark}

\newcounter{mymac@matlab}
\setcounter{mymac@matlab}{0}
\newcommand{\matlab}{MATLAB%
\ifnum\value{mymac@matlab}<1%
\textsuperscript{\textregistered}%
\setcounter{mymac@matlab}{1}%
\fi%
}
\newcommand{\mess}{\textsf{M-M.E.S.S.}}
\newcommand{\amd}{AMD}
% ---------Special math commands---------
\newcommand{\myparen}[1]{\left(#1\right)}

\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\spn}{span}	% span of vectors
\DeclareMathOperator{\sign}{sign}   % the sign function
\DeclareMathOperator{\ran}{range}
\DeclareMathOperator{\nul}{null}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\vecop}{vec}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclareMathOperator{\dom}{dom}
\newcommand{\rank}[1]{\ensuremath{\operatorname{rank}\!\myparen{#1}}}
\renewcommand{\d}{\,\mathrm{d}}		% differential
\renewcommand{\Re}[1]{\mathrm{Re}{\left(#1\right)}}   % real part
\renewcommand{\Im}[1]{\mathrm{Im}{\left(#1\right)}}   % imaginary part
\newcommand{\R}{\mathbb{R}}   % the real numbers
\newcommand{\TT}{{\ensuremath{\mkern-1.5mu\mathsf{T}}}} % real transpose

% norms
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\newcommand{\normF}[1]{\ensuremath{\norm{#1}_F}}
\def\normt#1{\|#1\|_{2}}

% ---------Standard notations---------
\newcommand{\eps}{\varepsilon}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\Rn}{\ensuremath{\R^{n}}}
\newcommand{\Rm}{\ensuremath{\R^{m}}}
\newcommand{\Rnm}{\ensuremath{\R^{n\times m}}}
\newcommand{\Rmm}{\ensuremath{\R^{m\times m}}}
\newcommand{\Rnn}{\ensuremath{\R^{n\times n}}}
\newcommand{\Rnr}{\ensuremath{\R^{n\times r}}}
\newcommand{\Rrr}{\ensuremath{\R^{r\times r}}}
\newcommand{\Rmr}{\ensuremath{\R^{m\times r}}}
\newcommand{\Rnk}{\ensuremath{\R^{n\times k}}}
\newcommand{\Rkk}{\ensuremath{\R^{k\times k}}}
\newcommand{\Rmk}{\ensuremath{\R^{m\times k}}}

\newcommand{\cA}{\ensuremath{\mathcal{A}}}
\newcommand{\cB}{\ensuremath{\mathcal{B}}}
\newcommand{\cC}{\ensuremath{\mathcal{C}}}
\newcommand{\cD}{\ensuremath{\mathcal{D}}}
\newcommand{\cE}{\ensuremath{\mathcal{E}}}
\newcommand{\cF}{\ensuremath{\mathcal{F}}}
\newcommand{\cG}{\ensuremath{\mathcal{G}}}
\newcommand{\cH}{\ensuremath{\mathcal{H}}}
\newcommand{\cI}{\ensuremath{\mathcal{I}}}
\newcommand{\cJ}{\ensuremath{\mathcal{J}}}
\newcommand{\cK}{\ensuremath{\mathcal{K}}}
\newcommand{\cL}{\ensuremath{\mathcal{L}}}
\newcommand{\cLvec}{\ensuremath{\cL_{\vecop}}}
\newcommand{\Pivec}{\ensuremath{\Pi_{\vecop}}}
\newcommand{\cM}{\ensuremath{\mathcal{M}}}
\newcommand{\cN}{\ensuremath{\mathcal{N}}}
\newcommand{\cO}{\ensuremath{\mathcal{O}}}
\newcommand{\cP}{\ensuremath{\mathcal{P}}}
\newcommand{\cQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\cR}{\ensuremath{\mathcal{R}}}
\newcommand{\cS}{\ensuremath{\mathcal{S}}}
\newcommand{\cT}{\ensuremath{\mathcal{T}}}
\newcommand{\cU}{\ensuremath{\mathcal{U}}}
\newcommand{\cV}{\ensuremath{\mathcal{V}}}
\newcommand{\cW}{\ensuremath{\mathcal{W}}}
\newcommand{\cX}{\ensuremath{\mathcal{X}}}
\newcommand{\cY}{\ensuremath{\mathcal{Y}}}
\newcommand{\cZ}{\ensuremath{\mathcal{Z}}}
%%%% \tilde letters
\newcommand{\tA}{\ensuremath{\widetilde{A}}}
\newcommand{\tB}{\ensuremath{\widetilde{B}}}
\newcommand{\tC}{\ensuremath{\widetilde{C}}}
\newcommand{\tD}{\ensuremath{\widetilde{D}}}
\newcommand{\tE}{\ensuremath{\widetilde{E}}}
\newcommand{\tF}{\ensuremath{\widetilde{F}}}
\newcommand{\tG}{\ensuremath{\widetilde{G}}}
\newcommand{\tH}{\ensuremath{\widetilde{H}}}
\newcommand{\tI}{\ensuremath{\widetilde{I}}}
\newcommand{\tJ}{\ensuremath{\widetilde{J}}}
\newcommand{\tK}{\ensuremath{\widetilde{K}}}
\newcommand{\tL}{\ensuremath{\widetilde{L}}}
\newcommand{\tM}{\ensuremath{\widetilde{M}}}
\newcommand{\tN}{\ensuremath{\widetilde{N}}}
\newcommand{\tO}{\ensuremath{\widetilde{O}}}
\newcommand{\tP}{\ensuremath{\widetilde{P}}}
\newcommand{\tQ}{\ensuremath{\widetilde{Q}}}
\newcommand{\tR}{\ensuremath{\widetilde{R}}}
\newcommand{\tS}{\ensuremath{\widetilde{S}}}
\newcommand{\tT}{\ensuremath{\widetilde{T}}}
\newcommand{\tU}{\ensuremath{\widetilde{U}}}
\newcommand{\tV}{\ensuremath{\widetilde{V}}}
\newcommand{\tW}{\ensuremath{\widetilde{W}}}
\newcommand{\tX}{\ensuremath{\widetilde{X}}}
\newcommand{\tY}{\ensuremath{\widetilde{Y}}}
\newcommand{\tZ}{\ensuremath{\widetilde{Z}}}
\newcommand{\tSigma}{\ensuremath{\widetilde{\Sigma}}}
\newcommand{\tgamma}{\ensuremath{\widetilde{\gamma}}}

%
\newcommand{\ta}{\ensuremath{\widetilde{a}}}
\newcommand{\tb}{\ensuremath{\widetilde{b}}}
\newcommand{\tc}{\ensuremath{\widetilde{c}}}
\newcommand{\td}{\ensuremath{\widetilde{d}}}
\newcommand{\te}{\ensuremath{\widetilde{e}}}
\newcommand{\tf}{\ensuremath{\widetilde{f}}}
\newcommand{\tg}{\ensuremath{\widetilde{g}}}
\newcommand{\tth}{\ensuremath{\widetilde{h}}}
\newcommand{\ti}{\ensuremath{\widetilde{i}}}
\newcommand{\tj}{\ensuremath{\widetilde{j}}}
\newcommand{\tk}{\ensuremath{\widetilde{k}}}
\newcommand{\tl}{\ensuremath{\widetilde{l}}}
\newcommand{\tm}{\ensuremath{\widetilde{m}}}
\newcommand{\tn}{\ensuremath{\widetilde{n}}}
\newcommand{\tto}{\ensuremath{\widetilde{o}}}
\newcommand{\tp}{\ensuremath{\widetilde{p}}}
\newcommand{\tq}{\ensuremath{\widetilde{q}}}
\newcommand{\tr}{\ensuremath{\widetilde{r}}}
\newcommand{\tss}{\ensuremath{\widetilde{s}}}
\newcommand{\ttt}{\ensuremath{\widetilde{t}}}
\newcommand{\tu}{\ensuremath{\widetilde{u}}}
\newcommand{\tv}{\ensuremath{\widetilde{v}}}
\newcommand{\tw}{\ensuremath{\widetilde{w}}}
\newcommand{\tx}{\ensuremath{\widetilde{x}}}
\newcommand{\ty}{\ensuremath{\widetilde{y}}}
\newcommand{\tz}{\ensuremath{\widetilde{z}}}
%%%% \hat letters
\newcommand{\hA}{\ensuremath{\widehat{A}}}
\newcommand{\hB}{\ensuremath{\widehat{B}}}
\newcommand{\hC}{\ensuremath{\widehat{C}}}
\newcommand{\hD}{\ensuremath{\widehat{D}}}
\newcommand{\hE}{\ensuremath{\widehat{E}}}
\newcommand{\hF}{\ensuremath{\widehat{F}}}
\newcommand{\hG}{\ensuremath{\widehat{G}}}
\newcommand{\hH}{\ensuremath{\widehat{H}}}
\newcommand{\hI}{\ensuremath{\widehat{I}}}
\newcommand{\hJ}{\ensuremath{\widehat{J}}}
\newcommand{\hK}{\ensuremath{\widehat{K}}}
\newcommand{\hL}{\ensuremath{\widehat{L}}}
\newcommand{\hM}{\ensuremath{\widehat{M}}}
\newcommand{\hN}{\ensuremath{\widehat{N}}}
\newcommand{\hO}{\ensuremath{\widehat{O}}}
\newcommand{\hP}{\ensuremath{\widehat{P}}}
\newcommand{\hQ}{\ensuremath{\widehat{Q}}}
\newcommand{\hR}{\ensuremath{\widehat{R}}}
\newcommand{\hS}{\ensuremath{\widehat{S}}}
\newcommand{\hT}{\ensuremath{\widehat{T}}}
\newcommand{\hU}{\ensuremath{\widehat{U}}}
\newcommand{\hV}{\ensuremath{\widehat{V}}}
\newcommand{\hW}{\ensuremath{\widehat{W}}}
\newcommand{\hX}{\ensuremath{\widehat{X}}}
\newcommand{\hY}{\ensuremath{\widehat{Y}}}
\newcommand{\hZ}{\ensuremath{\widehat{Z}}}
\newcommand{\hSigma}{\ensuremath{\widehat{\Sigma}}}
%
\newcommand{\ha}{\ensuremath{\widehat{a}}}
\newcommand{\hb}{\ensuremath{\widehat{b}}}
\newcommand{\hc}{\ensuremath{\widehat{c}}}
\newcommand{\hd}{\ensuremath{\widehat{d}}}
\newcommand{\he}{\ensuremath{\widehat{e}}}
\newcommand{\hf}{\ensuremath{\widehat{f}}}
\newcommand{\hg}{\ensuremath{\widehat{g}}}
\newcommand{\hth}{\ensuremath{\widehat{h}}}
\newcommand{\hi}{\ensuremath{\widehat{i}}}
\newcommand{\hj}{\ensuremath{\widehat{j}}}
\newcommand{\hk}{\ensuremath{\widehat{k}}}
\newcommand{\hm}{\ensuremath{\widehat{m}}}
\newcommand{\hn}{\ensuremath{\widehat{n}}}
\newcommand{\hto}{\ensuremath{\widehat{o}}}
\newcommand{\hp}{\ensuremath{\widehat{p}}}
\newcommand{\hq}{\ensuremath{\widehat{q}}}
\newcommand{\hr}{\ensuremath{\widehat{r}}}
\newcommand{\hs}{\ensuremath{\widehat{s}}}
\newcommand{\htt}{\ensuremath{\widehat{t}}}
\newcommand{\hu}{\ensuremath{\widehat{u}}}
\newcommand{\hv}{\ensuremath{\widehat{v}}}
\newcommand{\hw}{\ensuremath{\widehat{w}}}
\newcommand{\hx}{\ensuremath{\widehat{x}}}
\newcommand{\hy}{\ensuremath{\widehat{y}}}
\newcommand{\hz}{\ensuremath{\widehat{z}}}
\newcommand{\hgamma}{\ensuremath{\widehat{\gamma}}}
%%%% \check letters
\RequirePackage{mathabx}
\newcommand{\cgamma}{\ensuremath{\widecheck{\gamma}}}
%% bold math
\newcommand{\bm}[1]{\mathbf{#1}}
\newcommand{\bA}{\ensuremath{\bm{A}}}
\newcommand{\bB}{\ensuremath{\bm{B}}}
\newcommand{\bC}{\ensuremath{\bm{C}}}
\newcommand{\bD}{\ensuremath{\bm{D}}}
\newcommand{\bE}{\ensuremath{\bm{E}}}
\newcommand{\bF}{\ensuremath{\bm{F}}}
\newcommand{\bG}{\ensuremath{\bm{G}}}
\newcommand{\bH}{\ensuremath{\bm{H}}}
\newcommand{\bI}{\ensuremath{\bm{I}}}
\newcommand{\bJ}{\ensuremath{\bm{J}}}
\newcommand{\bK}{\ensuremath{\bm{K}}}
\newcommand{\bL}{\ensuremath{\bm{L}}}
\newcommand{\bM}{\ensuremath{\bm{M}}}
\newcommand{\bN}{\ensuremath{\bm{N}}}
\newcommand{\bO}{\ensuremath{\bm{O}}}
\newcommand{\bP}{\ensuremath{\bm{P}}}
\newcommand{\bQ}{\ensuremath{\bm{Q}}}
\newcommand{\bR}{\ensuremath{\bm{R}}}
\newcommand{\bS}{\ensuremath{\bm{S}}}
\newcommand{\bT}{\ensuremath{\bm{T}}}
\newcommand{\bU}{\ensuremath{\bm{U}}}
\newcommand{\bV}{\ensuremath{\bm{V}}}
\newcommand{\bW}{\ensuremath{\bm{W}}}
\newcommand{\bX}{\ensuremath{\bm{X}}}
\newcommand{\bY}{\ensuremath{\bm{Y}}}
\newcommand{\bZ}{\ensuremath{\bm{Z}}}
\newcommand{\ba}{\ensuremath{\bm{a}}}
\newcommand{\bb}{\ensuremath{\bm{b}}}
\newcommand{\bc}{\ensuremath{\bm{c}}}
\newcommand{\boldd}{\ensuremath{\bm{d}}}
\newcommand{\bolde}{\ensuremath{\bm{e}}}
\newcommand{\boldf}{\ensuremath{\bm{f}}}
\newcommand{\bg}{\ensuremath{\bm{g}}}
\newcommand{\bh}{\ensuremath{\bm{h}}}
\newcommand{\bj}{\ensuremath{\bm{j}}}
\newcommand{\bk}{\ensuremath{\bm{k}}}
\newcommand{\bl}{\ensuremath{\bm{l}}}
\newcommand{\boldm}{\ensuremath{\bm{m}}}
\newcommand{\bn}{\ensuremath{\bm{n}}}
\newcommand{\bo}{\ensuremath{\bm{o}}}
\newcommand{\bp}{\ensuremath{\bm{p}}}
\newcommand{\bq}{\ensuremath{\bm{q}}}
\newcommand{\br}{\ensuremath{\bm{r}}}
\newcommand{\bs}{\ensuremath{\bm{s}}}
\newcommand{\bt}{\ensuremath{\bm{t}}}
\newcommand{\bu}{\ensuremath{\bm{u}}}
\newcommand{\bv}{\ensuremath{\bm{v}}}
\newcommand{\bw}{\ensuremath{\bm{w}}}
\newcommand{\bx}{\ensuremath{\bm{x}}}
\newcommand{\by}{\ensuremath{\bm{y}}}
\newcommand{\bz}{\ensuremath{\bm{z}}}
\newcommand{\bnul}{\ensuremath{\bm{0}}}


% ---------Floating-point errors---------

% ---------Floating-point constants---------

% ---------For algorithms---------

% ---- pgf styles -----
\pgfplotscreateplotcyclelist{marks}{%
{color=blue, dashed, mark=x, mark options={solid}},
{color=black, dashed, mark=*, mark options={solid, fill=black!30}},
{color=blue!50, dashdotted, mark=triangle*, mark options={solid, fill=green}},
{color=red, dotted, mark=asterisk, mark options={solid}},
{color=brown,densely dotted, mark=square, mark options={solid}},
{color=blue,only marks,mark=diamond*,mark options={solid},fill=blue},
}

% ---------For rev---------
\newcommand*{\rev}[1]{{\color{brown}#1}}

